Integrating User Design and Formal Models within PVSio-Web

Creating formal models of interactive systems has wide reaching benefits, not only for verifying low-level correctness, but also as a tool for ensuring user interfaces behave logically and consistently. Despite this, tools for designing user experiences and tools for creating and working with formal models are typically distinctly separate systems. This work aims to bridge this divide by allowing the generation of state machine diagrams and formal models via a simple, interactive prototyping tool that mirrors the basic functionality of many modern digital prototyping applications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{95}
\providecommand{\publicationstatus}{P. Masci, R. Monahan, V. Prevosto (Eds.):  Formal\\
Integrated Development Environment 2018 (F-IDE 2018).\\
EPTCS 284, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.284.8}{10.4204/EPTCS.284.8}}
\pdfoutput=1

